Poisson measure as a spectral measure of a family of commuting selfadjoint operators, connected with some moment problem

It is proved that the Poisson measure is a spectral measure of some family of commuting selfadjoint operators acting on a space constructed from some generalization of the moment problem.

==> jinfo.tex <==
\jvolume{22}
\jyear{2016}
\jnumber{4}

